Evolving finite elements for advection diffusion with an evolving interface

The aim of this paper is to develop a numerical scheme to approximate evolving interface problems for parabolic equations based on the abstract evolving finite element framework proposed in (C M Elliott, T Ranner, IMA J Num Anal, 41:3, 2021, doi:10.1093/imanum/draa062). An appropriate weak formulation of the problem is derived for the use of evolving finite elements designed to accommodate a moving interface. Optimal order error bounds are proved for arbitrary order evolving isoparametric finite elements. The paper concludes with numerical results for a model problem verifying orders of convergence.

==> output/elliptic-order1-2d.tex <==
\begin{tabular}{ccccc}
\toprule
                     $h$ &              $L^2$ error & $H^1$ error & eoc($L^2$ error) & eoc($H^1$ error) \\
\midrule
               $1.00000$ & $4.19541 \times 10^{-1}$ &   $4.53786$ &              --- &              --- \\
$6.66667 \times 10^{-1}$ &                $1.15023$ &   $6.00618$ &        -2.487395 &        -0.691388 \\
$4.15188 \times 10^{-1}$ & $2.87831 \times 10^{-1}$ &   $3.31632$ &         2.925385 &         1.254195 \\
$2.05090 \times 10^{-1}$ & $1.30901 \times 10^{-1}$ &   $2.10520$ &         1.117181 &         0.644345 \\
$1.17237 \times 10^{-1}$ & $4.15358 \times 10^{-2}$ &   $1.13830$ &         2.052559 &         1.099457 \\
\bottomrule
\end{tabular}


==> output/elliptic-order1-3d.tex <==
\begin{tabular}{ccccc}
\toprule
                     $h$ &              $L^2$ error &             $H^1$ error & eoc($L^2$ error) & eoc($H^1$ error) \\
\midrule
               $1.12509$ & $8.87529 \times 10^{-1}$ & $1.08260 \times 10^{1}$ &              --- &              --- \\
$8.12325 \times 10^{-1}$ & $8.43674 \times 10^{-1}$ &               $9.85310$ &         0.155578 &         0.289102 \\
$6.25060 \times 10^{-1}$ & $7.25627 \times 10^{-1}$ &               $8.51027$ &         0.575191 &         0.559094 \\
$3.11922 \times 10^{-1}$ & $3.96853 \times 10^{-1}$ &               $5.72998$ &         0.868182 &         0.569074 \\
$1.59269 \times 10^{-1}$ & $1.24724 \times 10^{-1}$ &               $3.01830$ &         1.722008 &         0.953668 \\
\bottomrule
\end{tabular}


==> output/elliptic-order2-2d.tex <==
\begin{tabular}{ccccc}
\toprule
                     $h$ &              $L^2$ error &              $H^1$ error & eoc($L^2$ error) & eoc($H^1$ error) \\
\midrule
               $1.00000$ & $5.16377 \times 10^{-1}$ &                $4.92118$ &              --- &              --- \\
$6.66667 \times 10^{-1}$ & $2.04605 \times 10^{-1}$ &                $2.72634$ &         2.283193 &         1.456567 \\
$4.15188 \times 10^{-1}$ & $7.05885 \times 10^{-2}$ &                $1.42395$ &         2.247272 &         1.371593 \\
$2.05090 \times 10^{-1}$ & $8.39459 \times 10^{-3}$ & $3.85164 \times 10^{-1}$ &         3.019040 &         1.853890 \\
$1.17237 \times 10^{-1}$ & $1.22307 \times 10^{-3}$ & $1.09382 \times 10^{-1}$ &         3.444315 &         2.250922 \\
\bottomrule
\end{tabular}


==> output/elliptic-order2-3d.tex <==
\begin{tabular}{ccccc}
\toprule
                     $h$ & $L^2$ error & $H^1$ error & eoc($L^2$ error) & eoc($H^1$ error) \\
\midrule
               $1.12509$ &         nan &         nan &              --- &              --- \\
$8.12325 \times 10^{-1}$ &     0.47194 &    6.754057 &              --- &              --- \\
$6.25060 \times 10^{-1}$ &    0.197678 &    3.627296 &         3.320755 &         2.372254 \\
$3.11922 \times 10^{-1}$ &    0.026419 &     1.16411 &         2.895390 &         1.635071 \\
$1.59269 \times 10^{-1}$ &    0.003516 &    0.324048 &         3.000229 &         1.902553 \\
\bottomrule
\end{tabular}


==> output/elliptic-order3-2d.tex <==
\begin{tabular}{ccccc}
\toprule
                     $h$ &              $L^2$ error &              $H^1$ error & eoc($L^2$ error) & eoc($H^1$ error) \\
\midrule
               $1.00000$ & $2.57285 \times 10^{-1}$ &                $3.17243$ &              --- &              --- \\
$6.66667 \times 10^{-1}$ & $1.05259 \times 10^{-1}$ &                $1.42484$ &         2.204271 &         1.974113 \\
$4.15188 \times 10^{-1}$ & $6.50117 \times 10^{-3}$ & $2.01717 \times 10^{-1}$ &         5.879835 &         4.128214 \\
$2.05090 \times 10^{-1}$ & $6.58733 \times 10^{-4}$ & $4.13069 \times 10^{-2}$ &         3.246096 &         2.248511 \\
$1.17237 \times 10^{-1}$ & $5.16120 \times 10^{-5}$ & $6.15270 \times 10^{-3}$ &         4.553558 &         3.404823 \\
\bottomrule
\end{tabular}


==> output/elliptic-order3-3d.tex <==
\begin{tabular}{ccccc}
\toprule
                     $h$ &              $L^2$ error &              $H^1$ error & eoc($L^2$ error) & eoc($H^1$ error) \\
\midrule
               $1.12509$ & $4.29901 \times 10^{-1}$ &                $5.74274$ &              --- &              --- \\
$8.12325 \times 10^{-1}$ & $1.45173 \times 10^{-1}$ &                $3.19671$ &         3.333020 &         1.798517 \\
$6.25060 \times 10^{-1}$ & $3.16880 \times 10^{-2}$ &                $1.02034$ &         5.807928 &         4.357865 \\
$3.11922 \times 10^{-1}$ & $2.86216 \times 10^{-3}$ & $1.69628 \times 10^{-1}$ &         3.459039 &         2.581345 \\
$1.59269 \times 10^{-1}$ & $1.99219 \times 10^{-4}$ & $2.39944 \times 10^{-2}$ &         3.964720 &         2.909699 \\
\bottomrule
\end{tabular}

